Optical observations of the nearby galaxy IC342 with narrow band [SII] and H$\alpha$ filters. II - Detection of 16 Optically-Identified Supernova Remnant Candidates

We present the detection of 16 optical supernova remnant (SNR) candidates in the nearby spiral galaxy IC342. The candidates were detected by applying [SII]/H$\alpha$ ratio criterion on observations made with the 2 m RCC telescope at Rozhen National Astronomical Observatory in Bulgaria. In this paper, we report the coordinates, diameters, H$\alpha$ and [SII] fluxes for 16 SNRs detected in two fields of view in the IC342 galaxy. Also, we estimate that the contamination of total H$\alpha$ flux from SNRs in the observed portion of IC342 is 1.4%. This would represent the fractional error when the star formation rate (SFR) for this galaxy is derived from the total galaxy's H$\alpha$ emission.

==> astro.tex <==
\def\tg{\mathop{\rm tg}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}

\def\point#1{\hbox{\setbox7=\hbox to0.8em{\hfil.\hfil}%
\setbox8=\hbox to0.8em{\hfil$^{#1}$\hfil}%
\box7\kern-0.8em\box8}}

\def\dd{\point{\rm d}}
\def\hh{\point{\rm h}}
\def\mm{\point{\rm m}}
\def\ss{\point{\rm s}}

\def\oo{\point{\circ}}
\def\lll{\point{\prime}}
\def\uu{\point{\prime\prime}}




==> mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%yu-navodnik-pocetni
\def\navb{\char'134}                                      %yu-navodnik-krajnji
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} % Sasinci
\def\CJ{\' C} \def\cj{\' c} % Cicevac
\def\CH{\v C} \def\ch{\v c} % Xaxak
\def\Z{\v Z} \def\z{\v z} % Zuzemberk
\def\br{\break}



==> wncyr.tex <==
\def\rrmd{\font\tipo=wncyr12\tip}%
\def\rbfd{\font\tipo=wncyb12\tip}%
\def\rssd{\font\tipo=wncyss12\tip}%
\def\rrm{\font\tipo=wncyr10\tip}%
\def\rbf{\font\tipo=wncyb10\tip}%
\def\rit{\font\tipo=wncyi10\tip}%
\def\rss{\font\tipo=wncyss10\tip}%
\def\rsc{\font\tipo=wncysc10\tip}%
\def\rrmdev{\font\tipo=wncyr9\tip}%
\def\rbfdev{\font\tipo=wncyb9\tip}%
\def\ritdev{\font\tipo=wncyi9\tip}%
\def\rssdev{\font\tipo=wncyss9\tip}%
\def\rrmos{\font\tipo=wncyr8\tip}%
\def\rbfos{\font\tipo=wncyb8\tip}%
\def\ritos{\font\tipo=wncyi8\tip}%
\def\rssos{\font\tipo=wncyss8\tip}%
\def\rrmsev{\font\tipo=wncyr7\tip}%
\def\rbfsev{\font\tipo=wncyb7\tip}%
\def\ritsev{\font\tipo=wncyi7\tip}%
\def\tip{\relax\tipo\def\DD{\tipo\char'006}\def\dd{\tipo\char'016}% \tip
\def\DJ{\DD}\def\dj{\dd}% 
\def\ZZ{\tipo\char'021}\def\zz{\tipo\char'031}%
\def\Z{\ZZ}\def\z{\zz}%
\def\LJ{\tipo\char'001}\def\lj{\tipo\char'011}%
\def\NJ{\tipo\char'000}\def\nj{\tipo\char'010}%
\def\CC{\tipo\char'007}\def\cc{\tipo\char'017}%
\def\DZ{\tipo\char'002}\def\dz{\tipo\char'012}%
\def\XX{Q}\def\xx{q}%
\def\JJ{J}\def\jj{j}% 
\def\SS{X}\def\ss{x}%
\def\JA{\tipo\char'027}\def\ja{\tipo\char'037}%
\def\SC{W}\def\sc{w}%
\def\CJ{\CC}\def\cj{\cc}%
\def\CH{Q}\def\ch{q}%
\def\SH{X}\def\sh{x}%
% sch="x"; tvrdo i = "y"; ja = "j"; schtsch = "w"; tsch = "q"
\def\EE{\tipo\char'003}\def\ee{\tipo\char'013}% "e oborotnoe"
\def\JI{\tipo\char'022}\def\ji{\tipo\char'032}% rusko "j"
\def\JU{\tipo\char'020}\def\ju{\tipo\char'030}%
\def\M{\tipo\char'136}\def\m{\tipo\char'176}% meki znak
\def\TV{\tipo\char'137}\def\tv{\tipo\char'177}% tvrdi znak
\def\rnava{\tipo\char'074}\def\rnavb{\tipo\char'076}% ruski navodnici
\def\snava{\leavevmode\hbox{,\kern-0.06em,}}% yu-
\def\snavb{\tipo\char'134}}% navodnici
\def\br{\break}%



